Additive Invariants of Open Petri Nets

We classify all additive invariants of open Petri nets: these are $\mathbb{N}$-valued invariants which are additive with respect to sequential and parallel composition of open Petri nets. In particular, we prove two classification theorems: one for open Petri nets and one for monically open Petri nets (i.e. open Petri nets whose interfaces are specified by monic maps). Our results can be summarized as follows. The additive invariants of open Petri nets are completely determined by their values on a particular class of single-transition Petri nets. However, for monically open Petri nets, the additive invariants are determined by their values on transitionless Petri nets and all single-transition Petri nets. Our results confirm a conjecture of John Baez (stated during the AMS' 2022 Mathematical Research Communities workshop).

==> preamble.tex <==
%-------------------------------------------------------------------------
%
%   TABLE OF CONTENTS
%
%       A    general formatting packages 
%       B    collaborative editing 
%       C    graphics 
%       D    theorem environs and frames
%       E    mathematical symbols
%
%-------------------------------------------------------------------------

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~  A    general formatting packages  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%for the author formatting  
\usepackage[auth-sc]{authblk}

%%% In Header
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{rotating}

\usepackage{adjustbox}%for rescaling tikzcd diagrams

%tikz from John
\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{backgrounds,circuits,circuits.ee.IEC,shapes,fit,matrix}

\tikzstyle{simple}=[-,line width=2.000]
\tikzstyle{arrow}=[-,postaction={decorate},decoration={markings,mark=at position .5 with {\arrow{>}}},line width=1.100]
\pgfdeclarelayer{background}
\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{background,edgelayer,nodelayer,main}

\tikzstyle{none}=[inner sep=0pt]

\definecolor{lblue}{rgb}{0,250,255}
\tikzstyle{species}=[circle,fill=yellow,draw=black,scale=1.15]
\tikzstyle{transition}=[rectangle,fill=lblue,draw=black,scale=1.15]
\tikzstyle{inarrow}=[->, >=stealth, shorten >=.03cm,line width=1.5]
\tikzstyle{empty}=[circle,fill=none, draw=none]
\tikzstyle{inputdot}=[circle,fill=purple,draw=purple, scale=.25]
\tikzstyle{inputarrow}=[->,draw=purple, shorten >=.05cm]
\tikzstyle{simple}=[-,draw=purple,line width=1.000]

% We set up interlinked references.
\usepackage{url}
\usepackage{xcolor}
\definecolor{linkColor}{RGB}{156,78,13}
\usepackage{hyperref}
\hypersetup{
    colorlinks = true,
    allcolors = linkColor %set uniform color (def. above) for all links
    }
\usepackage{xspace}
% We set up nicer (postscript) fonts.
\usepackage{pslatex}

% We set up paragraphs without indentation
%\setlength\parindent{24pt}

% We set up version numbering of drafts
\usepackage{datetime}
\newdateformat{versiondate}{%
\THEMONTH\THEDAY}

% We set up AMS formatting, including seamless paragraph and theorem numbering.
\usepackage{amsthm}
%\usepackage[fleqn]{amsmath} % flush equations left
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{stix}

\usepackage{mathtools}

\usepackage{color}

%%% ADDED BY BEN: 
\usepackage{enumitem}
%\usepackage{fullpage} %%%%%%%%<<<<<<<<-----------
\usepackage{amsmath}
\usepackage{framed} %for framing of computational problems 

\usepackage{sectsty}
\allsectionsfont{\fontfamily{lmss}\selectfont}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~  B    collaborative editing  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

% Colored text for indicating changes
\def\DEBUG{true} %comment out to get rid of colors
\ifdefined\DEBUG{}
    \newcommand{\ben}[1]{{\color{teal}{#1}}}
    \newcommand{\sophie}[1]{{\color{purple}{#1}}}
    \newcommand{\jordy}[1]{{\color{olive}{#1}}}
    \newcommand{\layla}[1]{{\color{red}{#1}}}
    \newcommand{\sam}[1]{{\color{green}{#1}}}
    %
    \newcommand{\bovinenote}[1]{}
    \newcommand{\johnquestion}[1]{\hspace{-2cm}\textsc{\color{red}John} --- #1 \textsc{\color{red}end of question}}
    \newcommand{\tenkative}[1]{\hspace{-2cm}\textsc{\color{red}New Content} --- #1 \textsc{\color{red}end of new content}}
    %
    \newcommand{\FixPhrasingA}[1]{{\color{teal}#1}}
    \newcommand{\FixPhrasingB}[1]{{\color{purple}#1}}
    \newcommand{\FixPhrasingC}[1]{{\color{olive}#1}}
    \newcommand{\FixPhrasingD}[1]{{\color{red}#1}}
\else
    \newcommand{\ben}[1]{#1}
    \newcommand{\sophie}[1]{#1}
    \newcommand{\jordy}[1]{#1}
    \newcommand{\layla}[1]{#1}
    \newcommand{\sam}[1]{#1}
    %
    \newcommand{\FixPhrasingA}[1]{}
    \newcommand{\FixPhrasingB}[1]{}
    \newcommand{\FixPhrasingC}[1]{}
    \newcommand{\FixPhrasingD}[1]{}
    %
    \newcommand{\bovinenote}[1]{}
    \newcommand{\johnquestion}[1]{}
    \newcommand{\tenkative}[1]{}
\fi

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~  C    graphics  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

% We set up Tikz illustration scaling and commutative diagrams
\usepackage{pgf,tikz,environ}
\usepackage{quiver}
\usetikzlibrary{arrows}
\usetikzlibrary{cd}
\usetikzlibrary{positioning}
\usetikzlibrary{fadings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.pathmorphing}
\tikzset{snake it/.style={decorate, decoration=snake}}
\newcommand{\topline}
{%
  \tikz[remember picture,overlay] {%
    \draw[softGray] ([yshift=-1cm]current page.north west)
             -- ([yshift=-1cm,xshift=0.7\paperwidth]current page.north west);}
}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~  D    theorem environs and frames  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%--  special styles for bits of text inside theorems etc  ----------------

\newcommand{\defined}[1]{\textbf{#1}}

\renewcommand\qedsymbol{$\blacksquare$}

%--  shaded theorems etc  ------------------------------------------------

\definecolor{parchment}{RGB}{214, 204, 169}

\theoremstyle{plain}%-----------------------
%  
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{problem}[theorem]{Open Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question} 
 
\theoremstyle{definition}
%
\newtheorem{definition}[theorem]{Definition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{note}[theorem]{Note}
\newtheorem{aside}[theorem]{Aside}
\newtheorem{claim}[theorem]{Claim} 
\newtheorem{remark}[theorem]{Remark}

\usepackage{mdframed} %for shaded theorems and definitions
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{theorem}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{theorem*}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{corollary}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{lemma}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{problem}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{example}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{proposition}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{conjecture}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{definition}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{observation}
\surroundwithmdframed[hidealllines=true,backgroundcolor=parchment!40]{claim}

%--  unsure what this is  ------------------------------------------------

% SAM commented this out since not used

%\newcommand{\defproblem}[3]{
%	\vspace{1mm}
%	\noindent\fbox{
%		\begin{minipage}{0.96\textwidth}
%			\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1} &  \\ \end{tabular*}
%			{\bf{Input:}} #2 \\
%			{\bf{Question:}} #3
%		\end{minipage}
%	}
%	\vspace{1mm}
%}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~  E    mathematical symbols (TYPOGRAPHY)  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%--  modifiers  ----------------------------------------------------------

\newcommand{\Oh}{\mathcal{O}}

\newcommand{\pr}{^\prime}
\newcommand{\prpr}{^{\prime\prime}}

\newcommand{\dir}[1]{\overrightarrow{#1}}

%--  typesetting commands  -----------------------------------------------

\newcommand{\cc}[1]{\mathbf{#1}}
\newcommand{\typesetcategory}[1]{\cc{#1}}

\newcommand{\typesetoperator}[1]{\mathbf{#1}}
%
\DeclareMathOperator{\domain}{\typesetoperator{dom}}
\DeclareMathOperator{\codomain}{\typesetoperator{cod}}
\DeclareMathOperator{\mono}{\typesetoperator{Mono}}
\DeclareMathOperator{\sub}{\typesetoperator{Sub}}
\DeclareMathOperator{\homset}{\typesetoperator{Hom}}
\DeclareMathOperator{\obj}{\typesetoperator{Ob}}
\DeclareMathOperator{\morphisms}{\typesetoperator{Mor}}

\newcommand{\typesetproblem}[1]{\textsc{#1}}
%
\DeclareMathOperator{\p}{\typesetproblem{P}}
\DeclareMathOperator{\np}{\typesetproblem{NP}}
\DeclareMathOperator{\fpt}{\typesetproblem{FPT}}

%--  doublestruck and caligraphic upper letters (first batch)  -----------

\DeclareMathOperator{\Aa}{\mathcal{A}}  \DeclareMathOperator{\Ab}{\mathbb{A}}
\DeclareMathOperator{\Ba}{\mathcal{B}}  \DeclareMathOperator{\Bb}{\mathbb{B}}
\DeclareMathOperator{\Ca}{\mathcal{C}}  \DeclareMathOperator{\Cb}{\mathbb{C}}
\DeclareMathOperator{\Da}{\mathcal{D}}  \DeclareMathOperator{\Db}{\mathbb{D}}
\DeclareMathOperator{\Ea}{\mathcal{E}}  \DeclareMathOperator{\Eb}{\mathbb{E}}
\DeclareMathOperator{\Fa}{\mathcal{F}}  \DeclareMathOperator{\Fb}{\mathbb{F}}
\DeclareMathOperator{\Ga}{\mathcal{G}}  \DeclareMathOperator{\Gb}{\mathbb{G}}
\DeclareMathOperator{\Ha}{\mathcal{H}}  \DeclareMathOperator{\Hb}{\mathbb{H}}
\DeclareMathOperator{\Ia}{\mathcal{I}}  
\DeclareMathOperator{\Ja}{\mathcal{J}}  
\DeclareMathOperator{\Ka}{\mathcal{K}}  \DeclareMathOperator{\Kb}{\mathbb{K}}
\DeclareMathOperator{\La}{\mathcal{L}}  \DeclareMathOperator{\Lb}{\mathbb{L}}
\DeclareMathOperator{\Ma}{\mathcal{M}}  \DeclareMathOperator{\Mb}{\mathbb{M}}
\DeclareMathOperator{\Na}{\mathcal{N}}  \DeclareMathOperator{\Nb}{\mathbb{N}}
\DeclareMathOperator{\Oa}{\mathcal{O}}  \DeclareMathOperator{\Ob}{\mathbb{O}}
\DeclareMathOperator{\Pa}{\mathcal{P}}  \DeclareMathOperator{\Pb}{\mathbb{P}}
\DeclareMathOperator{\Qa}{\mathcal{Q}}  \DeclareMathOperator{\Qb}{\mathbb{Q}}
\DeclareMathOperator{\Ra}{\mathcal{R}}  \DeclareMathOperator{\Rb}{\mathbb{R}}
\DeclareMathOperator{\Sa}{\mathcal{S}}  \DeclareMathOperator{\Sb}{\mathbb{S}}
\DeclareMathOperator{\Ta}{\mathcal{T}}  \DeclareMathOperator{\Tb}{\mathbb{T}}
\DeclareMathOperator{\Ua}{\mathcal{U}}  \DeclareMathOperator{\Ub}{\mathbb{U}}
\DeclareMathOperator{\Va}{\mathcal{V}}  \DeclareMathOperator{\Vb}{\mathbb{V}}
\DeclareMathOperator{\Wa}{\mathcal{W}}  \DeclareMathOperator{\Wb}{\mathbb{W}}
\DeclareMathOperator{\Xa}{\mathcal{X}}  \DeclareMathOperator{\Xb}{\mathbb{X}}
\DeclareMathOperator{\Ya}{\mathcal{Y}}  \DeclareMathOperator{\Yb}{\mathbb{Y}}
\DeclareMathOperator{\Za}{\mathcal{Z}}  \DeclareMathOperator{\Zb}{\mathbb{Z}}

%--  doublestruck and caligraphic upper letters (second batch)  ----------

%\newcommand{\Aa}{\mathbb{A}}\newcommand{\aA}{\mathcal{A}}
%\newcommand{\Bb}{\mathbb{B}}\newcommand{\bB}{\mathcal{B}}
\newcommand{\Cc}{\mathbb{C}}\newcommand{\cC}{\mathcal{C}}
\newcommand{\Dd}{\mathbb{D}}\newcommand{\dD}{\mathcal{D}}
\newcommand{\Ee}{\mathbb{E}}\newcommand{\eE}{\mathcal{E}}
\newcommand{\Ff}{\mathbb{F}}\newcommand{\fF}{\mathcal{F}}
\newcommand{\Gg}{\mathbb{G}}\newcommand{\gG}{\mathcal{G}}
\newcommand{\Hh}{\mathbb{H}}\newcommand{\hH}{\mathcal{H}}
\newcommand{\Ii}{\mathbb{I}}\newcommand{\iI}{\mathcal{I}}
\newcommand{\Jj}{\mathbb{J}}\newcommand{\jJ}{\mathcal{J}}
\newcommand{\Kk}{\mathbb{K}}\newcommand{\kK}{\mathcal{K}}
\newcommand{\Ll}{\mathbb{L}}\newcommand{\lL}{\mathcal{L}}
\newcommand{\Mm}{\mathbb{M}}\newcommand{\mM}{\mathcal{M}}
\newcommand{\Nn}{\mathbb{N}}\newcommand{\nN}{\mathcal{N}}
\newcommand{\Oo}{\mathbb{O}}\newcommand{\oO}{\mathcal{O}}
\newcommand{\Pp}{\mathbb{P}}\newcommand{\pP}{\mathcal{P}}
\newcommand{\Qq}{\mathbb{Q}}\newcommand{\qQ}{\mathcal{Q}}
\newcommand{\Rr}{\mathbb{R}}\newcommand{\rR}{\mathcal{R}}
\newcommand{\Ss}{\mathbb{S}}\newcommand{\sS}{\mathcal{S}}
\newcommand{\Tt}{\mathbb{T}}\newcommand{\tT}{\mathcal{T}}
\newcommand{\Uu}{\mathbb{U}}\newcommand{\uU}{\mathcal{U}}
\newcommand{\Vv}{\mathbb{V}}\newcommand{\vV}{\mathcal{V}}
\newcommand{\Ww}{\mathbb{W}}\newcommand{\wW}{\mathcal{W}}
\newcommand{\Xx}{\mathbb{X}}\newcommand{\xX}{\mathcal{X}}
\newcommand{\Yy}{\mathbb{Y}}\newcommand{\yY}{\mathcal{Y}}
\newcommand{\Zz}{\mathbb{Z}}\newcommand{\zZ}{\mathcal{Z}}

%--  sans serif and frak lower letters  ----------------------------------

\newcommand{\sfa}{\mathsf{a}}\newcommand{\fra}{\mathcal{a}}
\newcommand{\sfb}{\mathsf{b}}\newcommand{\frb}{\mathcal{b}}
\newcommand{\sfc}{\mathsf{c}}\newcommand{\frc}{\mathcal{c}}
\newcommand{\sfd}{\mathsf{d}}\newcommand{\frd}{\mathcal{d}}
\newcommand{\sfe}{\mathsf{e}}\newcommand{\fre}{\mathcal{e}}
\newcommand{\sff}{\mathsf{f}}\newcommand{\frf}{\mathcal{f}}
\newcommand{\sfg}{\mathsf{g}}\newcommand{\frg}{\mathcal{g}}
\newcommand{\sfh}{\mathsf{h}}\newcommand{\frh}{\mathcal{h}}
\newcommand{\sfi}{\mathsf{i}}\newcommand{\fri}{\mathcal{i}}
\newcommand{\sfj}{\mathsf{j}}\newcommand{\frj}{\mathcal{j}}
\newcommand{\sfk}{\mathsf{k}}\newcommand{\frk}{\mathcal{k}}
\newcommand{\sfl}{\mathsf{l}}\newcommand{\frl}{\mathcal{l}}
\newcommand{\sfm}{\mathsf{m}}\newcommand{\frm}{\mathcal{m}}
\newcommand{\sfn}{\mathsf{n}}\newcommand{\frn}{\mathcal{n}}
\newcommand{\sfo}{\mathsf{o}}\newcommand{\fro}{\mathcal{o}}
\newcommand{\sfp}{\mathsf{p}}\newcommand{\frp}{\mathcal{p}}
\newcommand{\sfq}{\mathsf{q}}\newcommand{\frq}{\mathcal{q}}
\newcommand{\sfr}{\mathsf{r}}\newcommand{\frr}{\mathcal{r}}
\newcommand{\sfs}{\mathsf{s}}\newcommand{\frs}{\mathcal{s}}
\newcommand{\sft}{\mathsf{t}}\newcommand{\frt}{\mathcal{t}}
\newcommand{\sfu}{\mathsf{u}}\newcommand{\fru}{\mathcal{u}}
\newcommand{\sfv}{\mathsf{v}}\newcommand{\frv}{\mathcal{v}}
\newcommand{\sfw}{\mathsf{w}}\newcommand{\frw}{\mathcal{w}}
\newcommand{\sfx}{\mathsf{x}}\newcommand{\frx}{\mathcal{x}}
\newcommand{\sfy}{\mathsf{y}}\newcommand{\fry}{\mathcal{y}}
\newcommand{\sfz}{\mathsf{z}}\newcommand{\frz}{\mathcal{z}}
